FEABench: Evaluating Language Models on Multiphysics Reasoning Ability

Building precise simulations of the real world and invoking numerical solvers to answer quantitative problems is an essential requirement in engineering and science. We present FEABench, a benchmark to evaluate the ability of large language models (LLMs) and LLM agents to simulate and solve physics, mathematics and engineering problems using finite element analysis (FEA). We introduce a comprehensive evaluation scheme to investigate the ability of LLMs to solve these problems end-to-end by reasoning over natural language problem descriptions and operating COMSOL Multiphysics$^\circledR$, an FEA software, to compute the answers. We additionally design a language model agent equipped with the ability to interact with the software through its Application Programming Interface (API), examine its outputs and use tools to improve its solutions over multiple iterations. Our best performing strategy generates executable API calls 88% of the time. LLMs that can successfully interact with and operate FEA software to solve problems such as those in our benchmark would push the frontiers of automation in engineering. Acquiring this capability would augment LLMs' reasoning skills with the precision of numerical solvers and advance the development of autonomous systems that can tackle complex problems in the real world. The code is available at https://github.com/google/feabench

==> workshop_contents/abstract.tex <==
Building precise simulations of the real world and using numerical methods to solve quantitative problems is an essential task in engineering and physics. We present FEABench, a benchmark to evaluate the ability of language models (LLMs) and LLM agents to simulate and solve physics, mathematics and engineering problems using finite element analysis (FEA) software. We introduce a multipronged evaluation scheme to investigate the ability of LLMs to solve these problems using \comsol. We further design an LLM agent equipped with the ability to interact with the software through its Application Programming Interface (API), examine its outputs and use tools to improve its solution over several iterations. Our best performing strategy generates executable API calls \cready{88\%} of the time. However, this benchmark still proves to be challenging enough that the LLMs and agents we tested were not able to completely and correctly solve any problem. LLMs that can successfully interact with and operate FEA software to solve problems such as those in our benchmark would push the frontiers of automation in engineering. Acquiring this capability would augment LLMs' reasoning skills with the precision of numerical solvers and advance the development of autonomous systems that can tackle complex problems in the real world.

==> workshop_contents/agent_long.tex <==
\begin{figure}[h]
\includegraphics[width=\textwidth]{figs/agent.pdf}
\caption{An overview of the agent and environment design, and the steps involved returning the next solution.}
\label{fig:agent}
\end{figure}
% That is already the case since the tables above it have nothing to do with the agent (they're for different models and the direct prompting setup). The Agent results are in Tab4-5.


% I initially set the color scheme so the steps happening in the same agent have the same color. But it's probably redundant since I also explicitly say Step N: <Agent>
% I get it that each color is a different agent, but the figure might need some more arrows. or sort of some other spatial arrangement. But it's not critical. You can work on it afterwards.

%connecting outputs of the previous step to the next?

We design a nested multi-agent system and an environment for the agent to interact with, in order to improve its solution. The environment includes the \comsol API, as well as tools that contain information relevant to correcting a problem. Each agent has a specific role and input context.

\textsc{ControllerAgent}: This is the overall agent that tries to solve the problem description by generating solutions, interacting with the API and calling subagents that return better solutions.\newline
\textbf{Input Context}: Problem description.\newline
\textbf{Components}: Evaluator, ControllerSubAgent\newline
\textbf{Working}: This samples an initial population of N(=20) solutions. Each solution is evaluated by the Evaluator. A fitness score, between 0 and 2, is computed for each solution, using the following formula: Executability + ExportSuccessful where ExportSuccessful is 1 if the solution exported a non-empty table and had executability above 90\% and 0 if not. The controller agent tracks a set of best replies. This will include at least B(=1) solution, as well as all solutions that successfully exported a non-empty table. This agent also determines the context to be sent to the CorrectorSubAgent, using the following algorithm:
\begin{itemize}\itemsep0em
    \item Solution to iterate on: We use an iteration criterion based inspired by the Markov Chain Monte Carlo (MCMC) acceptance criterion. The solution to iterate on (rendered in the prompt to the CorrectorSubAgent as “CURRENT CODE”) is a) the last solution if the last solution has equal fitness as the best solution, or b) if a random float between [0, 1] is less than $\alpha = \frac{Last\_Fitness}{Best\_Fitness}$, it is the last solution, else the best solution.
    \item ExecutionHistory: The best solutions, if not already used in context upto a maximum of \change{3} best solutions.
    \item BadSolutions: The last N\_bad(=1) replies, if not already in context. \newline
\end{itemize}

\definecolor{lm}{HTML}{5954a4}

\begin{figure}[t]
\includegraphics[width=\textwidth]{figs/tool_demo.pdf}
\caption{The execution feedback (\textit{left}) is passed to the ToolLookupAgent, that calls \textbf{\textit{tools}} and returns their combined output. {\color{lm} \textbf{Violet}} on the \textit{right}, denotes the arguments to the ToolCalls, that the ToolLookupAgent generates in order to call the tools.}
\label{fig:tool_demo}
\end{figure}


\textsc{Evaluator}: Returns the feedback for a solution in a `score' dictionary.\newline
\textbf{Input Context}: Solution. \newline
\textbf{Working}: The evaluator combines execution feedback with subjective feedback from an LM. This design choice is motivated by the fact that API messages alone don't have any information about the exported table, or about information that might be inconsistent with the problem, or missing in the solution. The evaluator executes the parsed solution in the API, and stores the API messages as well as the Executability. If the Executability exceeds a threshold of 90\%, the VerifierLM examines the code as well as the table in `output.txt' and returns feedback on what changes need to be made in the code. In order to do this, the VerifierLM sets an analytical guess for what the solution should be at the onset of the problem, and compares the exported table with this guess each time it evaluates a solution. The API feedback provides a signal on \textit{correctness} and the VerifierLM provides a signal on \textit{completeness}. Note, this evaluator is not provided the ground truth answer.  \newline

\textsc{CorrectorSubagent}: This returns the next / corrected solution.\newline
\textbf{Input Context}: Problem description, Current Code and Feedback, Execution History\newline
\textbf{Components}: ToolLookupAgent\newline
\textbf{Working}: This calls the ToolLookupAgent and retrieves its reply. It then adds this reply to the rest of the context received from the ControllerAgent to propose the next solution.

\textsc{ToolLookupAgent:} This calls tools and returns the information retrieved from them. \newline
\textbf{Input Context}: Feedback (\fref{fig:tool_demo}) \newline 
\textbf{Components}: ToolRegistry\newline
\textbf{Working}: The LM is shown the tool descriptions as well as the input context and must return a list of tool calls, which are structured classes consisting of the tool name and its arguments. We use the Langfun interface for this\citep{Peng_Langfun_2023}. This is parsed and used to call the tools with their respective arguments. If the parsing fails, the ToolLookupAgent returns an empty reply.
If successful, each tool is called with its arguments and the replies are concatenated. All tools are designed so as to return strings, which can be injected into the prompt. The tools in the registry are:
\begin{enumerate}\itemsep0em
    \item \textsc{QueryPhysicsInterfaces}: \textbf{Args:} None. Returns the list of valid physics interfaces.
    \item \textsc{QueryPhysicsFeatures}: \textbf{Args:} `interface' [Optional]
    Returns the list of features under `interface' if interface is provided or is a valid interface. Else, returns the entire interface to feature mapping.
    \item \textsc{QueryModelTreeProperties}: \textbf{Args:} `path'. Returns the properties under the node corresponding to path.
    \item \textsc{RetrieveAnnotatedSnippets}: \textbf{Args:} branch, query. This consists of an annotated library of code description $\rightarrow$ code snippet pairs, organized by branch (geometry, physics etc). This returns the 3 description / code snippet pairs closest to the query.
\end{enumerate}

% \begin{table}[h]
% \centering
% \caption{Code Metrics: Fixed: Gemini 1.5 Pro $|$Varying tasks, prompts, agent setting.}
% \begin{tabular}{p{1.1in}p{.7in}p{0.9in}p{0.9in}p{1in}}
% \toprule
% Description & Executability & Model Tree Score & Code Similarity Score & \# LM Judged Export \\
% \midrule
% ModelSpecs & 0.65$\pm$0.04 & 0.48$\pm$0.06 & 0.22$\pm$0.03 & 0/15 \\
% Plan & 0.58$\pm$0.04 & 0.44$\pm$0.04 & \textbf{0.25}$\pm$0.03 & 0/15 \\
% ModelSpecs+PhyDoc & 0.67$\pm$0.04 & 0.55$\pm$0.07 & 0.18$\pm$0.03 & 1/15 \\
% Plan+PhyDoc & 0.60$\pm$0.04 & 0.55$\pm$0.05 & \textbf{0.25}$\pm$0.03 & 1/15 \\
% ModelSpecs +Multi-Turn Agent & \textbf{0.92}$\pm$0.02 & \textbf{0.62}$\pm$0.07 & 0.18$\pm$0.03 & \textbf{5/15} \\
% \bottomrule
% \end{tabular}
% \vspace{0.1cm}
% \caption{Physics Metrics: Fixed: Gemini 1.5 Pro $|$Varying tasks, prompts, agent setting.}
% \begin{tabular}{p{1.1in}p{.75in}p{.6in}p{.6in}p{.7in}p{.7in}}
% \toprule
% Description & Interface Factuality & Interface Recall & Feature Recall & Feature Dimension & Feature Property Recall \\
% \midrule
% ModelSpecs & 0.54$\pm$0.14 & 0.46$\pm$0.14 & 0.54$\pm$0.12 & 0.69$\pm$0.16 & 0.20$\pm$0.10 \\
% Plan & 0.42$\pm$0.15 & 0.42$\pm$0.15 & 0.49$\pm$0.13 & 0.83$\pm$0.17 & 0.25$\pm$0.10 \\
% ModelSpecs +PhyDoc & \textbf{1.0}$\pm$0.0 & \textbf{0.86}$\pm$0.10 & 0.63$\pm$0.11 & 0.75$\pm$0.13 & 0.20$\pm$0.11 \\
% Plan +PhyDoc & 0.73$\pm$0.12 & 0.57$\pm$0.14 & 0.70$\pm$0.11 & \textbf{0.90}$\pm$0.10 & 0.25$\pm$0.11 \\
% ModelSpecs +Multi-Turn AgentEvolveMCMC-like & \textbf{1.0}$\pm$0.0 & 0.71$\pm$0.12 & \textbf{0.77}$\pm$0.11 & \textbf{0.90}$\pm$0.10 & \textbf{0.33}$\pm$0.12 \\
% \bottomrule
% \end{tabular}
% \end{table}



% \subsection{Qualitative Demonstration of a Single Step}



% \section{Fuzzy set and Fine-tuning?}
% \todo{For the agent stuff: it would be nice if we could add a video with the evolution of the model tree and screenshots of the built version of the comsol code in the GUI. (As a demo)}



==> workshop_contents/benchmain_only_res.tex <==
%This contains results without references to FEABench Large.
\begin{table}[!h]
\begin{small}
\centering
\caption{Code Metrics: Comparison on \model across LLMs.}
\label{tab:compare_models}
\begin{tabular}{p{1.2in}p{.7in}p{.9in}p{.9in}p{1in}}
\toprule
Experiment & Executability & Model Tree Score & Code Similarity & Valid Target \\
\midrule
Claude 3.5 Sonnet \citep{claude} & \textbf{0.79}$\pm$0.03 & \textbf{0.69}$\pm$0.07 & \textbf{0.19}$\pm$0.03 & \textbf{1}/15 \\
GPT-4o \citep{gpt4orelease} & 0.78$\pm$0.03 & 0.56$\pm$0.06 & 0.17$\pm$0.03 & 0/15 \\
Gemini-1.5-Pro \citep{reid2024gemini} & 0.60$\pm$0.05 & 0.46$\pm$0.07 & 0.17$\pm$0.03 & 0/15 \\
\bottomrule
\end{tabular}
\vspace{0.1cm}
\caption{Physics Metrics: Comparison on \model across LLMs.}
\label{tab:compare_models2}
\begin{tabular}{p{1.1in}p{.75in}p{.6in}p{.6in}p{.7in}p{.7in}}
\toprule
Experiment & Interface \mbox{Factuality} & Interface Recall & Feature \mbox{Recall} & Feature \mbox{Property} Recall & Feature Dimension \\
\midrule
Claude 3.5 Sonnet & \textbf{0.85}$\pm$0.10 & \textbf{0.71}$\pm$0.13 & \textbf{0.80}$\pm$0.10 & \textbf{0.22}$\pm$0.10 & \textbf{0.95}$\pm$0.05 \\
GPT-4o & 0.79$\pm$0.11 & 0.64$\pm$0.13 & 0.55$\pm$0.12 & \textbf{0.22}$\pm$0.11 & \textbf{0.95}$\pm$0.05 \\
Gemini-1.5-Pro & 0.54$\pm$0.14 & 0.43$\pm$0.14 & 0.39$\pm$0.10 & 0.15$\pm$0.09 & 0.86$\pm$0.14 \\
\bottomrule
\end{tabular}
\end{small}
\end{table}

\begin{table}[h]
\begin{small}
\centering
\caption{Code Metrics: Comparison across tasks, prompts and agents.}
\label{tab:compare_ongem}
\begin{tabular}{p{1.8in}p{.7in}p{.7in}p{.7in}p{.7in}}
\toprule
Experiment & Executability & Model Tree Score & Code \mbox{Similarity} & Valid Target \\
\midrule
\model: One-Shot & 0.60$\pm$0.05 & 0.46$\pm$0.07 & 0.17$\pm$0.03 & 0/15 \\
\model: PhyDoc In-Context & 0.62$\pm$0.05 & 0.58$\pm$0.07 & 0.15$\pm$0.02 & 1/15 \\
\model: Multi-Turn Agent & \textbf{0.88}$\pm$0.03 & 0.56$\pm$0.08 & 0.17$\pm$0.03 & \textbf{2}/15 \\
\midrule
\plan: One-Shot & 0.54$\pm$0.03 & 0.39$\pm$0.03 & \textbf{0.21}$\pm$0.03 & 0/15 \\
\plan: PhyDoc In-Context & 0.59$\pm$0.05 & \textbf{0.59}$\pm$0.06 & 0.20$\pm$0.02 & 0/15 \\
\bottomrule
\end{tabular}
\vspace{0.1cm}
\caption{Physics Metrics: Comparison across tasks, prompts and agents.}
\label{tab:compare_ongem2}
\begin{tabular}{p{1.7in}p{.5in}p{.5in}p{.5in}p{.65in}p{.6in}}
\toprule
Experiment & Interface Factuality & Interface Recall & Feature Recall & Feature \mbox{Property} Recall & Feature \mbox{Dimension} \\
\midrule
\model: One-Shot & 0.54$\pm$0.14 & 0.43$\pm$0.14 & 0.39$\pm$0.10 & 0.15$\pm$0.09 & 0.86$\pm$0.14 \\
\model: PhyDoc In-Context & \textbf{1.00}$\pm$0.00 & 0.71$\pm$0.13 & 0.48$\pm$0.10 & 0.08$\pm$0.07 & 0.59$\pm$0.16 \\
\model: Multi-Turn Agent & 0.93$\pm$0.07 & \textbf{0.79}$\pm$0.11 & \textbf{0.75}$\pm$0.09 & 0.24$\pm$0.10 & 0.89$\pm$0.07 \\
\midrule
\plan: One-Shot & 0.38$\pm$0.14 & 0.36$\pm$0.13 & 0.43$\pm$0.11 & \textbf{0.32}$\pm$0.11 & 0.79$\pm$0.15 \\
\plan: PhyDoc In-Context & 0.85$\pm$0.10 & 0.57$\pm$0.14 & 0.47$\pm$0.11 & 0.13$\pm$0.07 & \textbf{0.93}$\pm$0.07 \\
\bottomrule
\end{tabular}
\end{small}
\end{table}

\paragraph{Comparison across LLMs} Our baseline experiment queries \cready{different} frontier LLMs with a one-shot prompt (see \aref{app: prompts}). \tref{tab:compare_models} records the means and standard errors on the means across problems. Mean executability is in the range \cready{0.60-0.79}, implying that the LLMs are familiar with the higher-level grammar and syntax of \comsol API code. However, they are prone to hallucinating the choice of interface (factuality between \cready{$[0.54-0.85]$}). This is likely a significant contributor to the non-executable lines because an invalid interface renders all physics lines of code under this interface invalid. Claude 3.5-Sonnet has the best performance in the baseline setting. See \aref{app:qual} for a qualitative analysis.

==> workshop_contents/conc.tex <==
Our benchmark seeks to inspire rigorous evaluations of the capabilities of LLMs on solving problems that require simulating physical phenomena in the real world and performing numerical analysis. Such problems are ubiquitous in science and engineering, and solving them requires synthesizing reasoning over the physics domain with the ability to leverage numerical analysis software such as FEA. Our dataset serves as a novel testbed to evaluate the ability of LLMs to interact with feedback from an execution environment, correctly analyze and attribute errors and correct them. Future directions include devising agent strategies that boost performance, \change{adding more benchmark problems}, increasing problem complexity \change{such as working with more complex geometries, and examining whether performance improves by leveraging GUI visual information}. An LLM system that can successfully master FEA software would unlock the ability to solve a range of real-world engineering and physics problems. 

==> workshop_contents/data.tex <==
\change{The benchmark problems are derived from tutorials in the \comsol Application Gallery \cite{tuts} which are often based on established validation problems or other sources \citep{melnik2003bandstructures, national1990standard}. The input is a problem description describing a problem with a specific target quantity that needs to be computed (\fref{fig:schema}). The problems span a range of real world / mathematical systems including the dynamics of a Lorenz attractor, heat transfer, and a Bragg reflector. Each entry consists of the following main fields: (1) \textbf{Model Specifications:} A condensed yet fully-specified description of the problem, and the physics / boundary conditions. This description is unambiguous in terms of details such as material properties or dimensions. (2) \textbf{Selection Information:} An engineer would rely on visual information from the \change{Graphical User Interface (GUI)} (\fref{fig:comsol_pic}) for spatial information, particularly the numerical representation of geometrical entities, like points or boundaries. Since the agents do not have visual access to the GUI, we augment the model specifications with this information, to supply the model with the necessary representation of spatial information in the GUI. This information will be valid as long as the agent chooses to construct the geometry in a manner reasonably similar to how the ground truth (GT) geometry was created. (3) \textbf{Plan:} An explicit step-by-step description in natural language of the steps to be followed to solve the problem using \comsol. Either of the following comprise \change{self-sufficient tasks for the agent to solve: a) Model Specifications + Selection Information (designated \textbf{ModelSpecs}), or b) Plan (\textbf{Plan}).} (4) \textbf{Target Description:} A brief phrase describing the quantity that needs to be computed. (5) \textbf{Target Value:} The correct value of the target physical quantity. \cready{Note, the target values are expected to be largely independent of the choice of modeling software.} (6) \textbf{Ground Truth Code: } Ground truth code, that if executed, is able to successfully solve the problem and export the target value to a file. (7) \textbf{Model Tree: } Executing \comsol calls essentially build a model that can be regarded as modifying a tree with certain predefined `branches' such as `geometry' and `physics'. The model generated by executing code can thus be represented in a condensed form as a model tree (see \aref{app: example_bench} for an example). Converting a tutorial to a benchmark problem requires ensuring that a verifiable artifact (the target) can be derived from it, generating inputs and ensuring they have all the information needed to solve the problem, generating the GT solution and verifying that it exports the correct target value (\aref{A: Dataset})}.


==> workshop_contents/eval.tex <==
Our evaluation metrics measure the correctness of the solution, even when a target value could not be exported, (\tref{tab:metrics_2}). These additional metrics offer the advantage of being continuous, unlike the relative error, which can only be computed if the solution exported a valid target value. Metrics denoted by \textsuperscript{\textdagger} require execution. We delineate the metrics, and the facets they probe here: (1) \textbf{Executability\textsuperscript{\textdagger}:} `Correct' (executable) lines as a fraction of parsed API calls in an LLM solution. (2) \textbf{Model Tree Score\textsuperscript{\textdagger}:} Similarity score between the LLM code's model tree and the GT tree. This normalized so that a solution with no lines of code is scored 0. If equivalent to the GT code, it would be 1. This measures the \textit{alignment} of the model's solution path with a successful path. (3) \textbf{Code Similarity Score: }Similarity score between the solution and the GT code. While this also measures alignment with the GT solution, two different code blocks could generate equivalent model subtrees. \cready{We mainly report this metric for completeness, and to motivate the need for the domain-specific metrics we introduce here.}
(4) \textbf{Physics Metrics:} The code is a basis to represent the actions the LM takes to model the problem. Since the physics block is the most challenging (\fref{fig:blockwise}), we additionally analyze the LLM's physics action sequence by parsing and evaluating the physics commands. The most basic physics action sequence involves: Create Interface \change{(eg: HeatTransfer)} $\rightarrow$ Create Feature under Interface \change{(eg: TemperatureBoundary)} $\rightarrow$ Modify Feature Properties \change{(eg: T0, to set a temperature)}. Our Physics Metrics include (a) \textit{Interface Factuality}: How many defined interfaces were \textit{not} hallucinated? (b) \textit{Interface / Feature / Feature Property Recall}: How many interfaces / features / feature properties created / modified by the GT solution were also in the LLM solution? (c) \textit{Feature Dimension:} For features created by both, does the feature's spatial dimension match? \cready{Some nested physics metrics, such as `Feature Dimension' might not be valid for a specific problem, in case there was no matching feature between the ground truth and the LLM code: we mask out these problems while computing the means for that specific metric.} (5) \textbf{Target Relative Error\textsuperscript{\textdagger}}: There are various ways in which exporting the correct value may fail: a) the code fails to export b) it exports an `empty' table or, c) it exports an incorrect table, such as a default value or the wrong quantity. We ask an LLM to check that the exported table matches the target description and that the exported quantity is not a default or a value reproduced as is from the problem description, and to parse the response, if so. \textbf{Valid Target} is the number of problems in the benchmark for which the LLM successfully judges the exported table to be valid. We then compute the relative error between the last value in the exported table and the GT answer. \textbf{ Relative Error $\vert$ Strict} computes the mean relative error only over problems for which Valid Export is True, \textsc{AND} the relative error is less than 10\%. Relative Error $\vert$ Strict is our key metric for whether the LLM truly solved a problem.


==> workshop_contents/intro_math.tex <==
Several works have demonstrated the significant potential of large language models (LLMs) on analytical mathematical and scientific reasoning  \citep{lewkowycz2022solving, yang2024leandojo,hendrycks2021measuring,rein2023gpqa,pan2024quantum,trinh2024solving}, and on programming tasks in general-purpose languages like Python \citep{chen2021evaluating,tian2024scicode,yang2024swe}. However, many quantitative tasks that are the cornerstone of engineering and scientific workflows require numerical analysis performed with sophisticated computational modeling software. For example, the development of a modern smartphone requires detailed modeling of the mechanical, thermal, and electrical behaviors of its many subcomponents. Finite element analysis (FEA) \cite{courant1994variational} is the approach typically used. This involves approximating the partial differential equations that describe the physical behavior of a system by building discretizations (or meshes) over geometries. This is then solved until convergence using numerical solvers. The vast relevance of FEA to domains like mechanical, biomedical and aerospace engineering, optics, and fluid dynamics has given rise to software such as Ansys\reg \citep{ansys}, Abaqus\reg { FEA} \citep{abaqus}, and \comsol \citep{comsol,multiphysics1998introduction}, that are indispensable to modelling complex systems with the interplay of non-trivial geometries, and multiple physical phenomena. 

% These tasks usually cannot be solved analytically and would require significantly more effort to model from scratch with non-specialized tools in mainstream languages like C++ or Python.

In this paper, we begin to bridge this gap by examining the ability of LLMs to solve problems using finite element analysis (FEA) by generating Java API calls. This task requires reasoning over the problem and the ability to successfully operate the software. We selected \comsol because it supports a wide range of physics models and can be applied to applied mathematics problems involving optimization or differential equations, to problems involving complex geometries. Because the FEA workflow is relatively canonical, the reasoning approach for modeling is similar to other FEA software, and all problems typically share a conceptual breakdown into a sequence of blocks that involve defining (1) Geometry, (2) Material properties, (3) Physics, (4) Meshing (5) \change{Numerical Analysis and Solver settings, and (6) Postprocessing (details in \aref{app: codeblocks})}. \comsol Version 6.1 is used in this work.

Our contributions are the following: We create a benchmark of \cready{15} quantitatively verifiable problems. These problems require numerical methods to solve, and the target values are expected to be largely independent of the modeling software.
% i.e. if the LM is able to generate the code to solve the problem correctly, it will export a table containing the desired target value to a file when executed. We additionally define two versions of the task, to probe different versions of task complexity and design a multi-score evaluation strategy to probe different facets of distance to the correct answer. 
We measure different state-of-the-art LLMs on their performance with a multi-score evaluation strategy. \omitifnoagent{Finally, we design a multi-turn LLM agent that interacts with the API and improves upon its answers over several iterations and examine its performance.}

==> workshop_contents/owa_data.tex <==
The benchmark problems are derived from tutorials in the \comsol Application Gallery \cite{tuts} which are often based on established validation problems or other sources \citep{melnik2003bandstructures, national1990standard}. The input is a problem description describing a problem with a specific target quantity that needs to be computed (\fref{fig:schema}). The problems span a range of real world / mathematical systems including the dynamics of a Lorenz attractor, heat transfer, and a Bragg reflector. Each entry consists of the following main fields:
\begin{enumerate}
\item \textbf{Model Specifications:} A condensed yet fully-specified description of the problem, and the physics / boundary conditions. This description is unambiguous in terms of details such as material properties or dimensions.
\item \textbf{Selection Information:} An engineer would rely on visual information from the \change{Graphical User Interface (GUI)} (\fref{fig:comsol_pic}) for spatial information, particularly the numerical representation of geometrical entities, like points or boundaries. Since the agents do not have visual access to the GUI, we augment the model specifications with this information, to supply the model with the necessary representation of spatial information in the GUI. This information will be valid as long as the agent chooses to construct the geometry in a manner reasonably similar to how the ground truth (GT) geometry was created. 
\item \textbf{Plan:} An explicit step-by-step description in natural language of the steps to be followed to solve the problem using \comsol. Either of the following comprise \change{self-sufficient tasks for the agent to solve: a) Model Specifications + Selection Information (designated \textbf{ModelSpecs}), or b) Plan (\textbf{Plan}).} 
\item \textbf{Target Description:} A brief phrase describing the quantity that needs to be computed. 
\item \textbf{Target Value:} The correct value of the target physical quantity. 
\item \textbf{Ground Truth Code: } Ground truth code, that if executed, is able to successfully solve the problem and export the target value to a file. 
\item \textbf{Model Tree: } Executing \comsol calls essentially build a model that can be regarded as modifying a tree with certain predefined `branches' such as `geometry' and `physics'. The model generated by executing code can thus be represented in a condensed form as a model tree (see \aref{app: example_bench} for an example). Converting a tutorial to a benchmark problem requires ensuring that a verifiable artifact (the target) can be derived from it, generating inputs and ensuring they have all the information needed to solve the problem, generating the GT solution and verifying that it exports the correct target value (\aref{A: Dataset}).
\end{enumerate}

==> workshop_contents/owa_longerres.tex <==
\cready{
\paragraph{Explicit natural language instructions don't always help.} We fix the LLM to Gemini-1.5-Pro and examine whether the \plan task is easier. The comparison between task versions is of interest since both demand slightly different skills. For a person attempting to solve this task, \model requires the individual to both \textit{infer }implicit engineering and physical reasoning decisions to be made (e.g.: for the problem in \fref{fig:schema}, the LLM needs to infer that the correct representation of a cylinder's 2D cross-section is a rectangle) and further translate this to valid API calls. \plan explicitly describes all steps to be followed in natural language and requires the LLM to only \textit{translate} the steps describing interactions with the GUI to valid calls. The comparison between the two tasks offers one way to decouple the difficulty arising from making correct modelling decisions from translating the decisions into calls with the correct syntax. If an LLM fared poorly at making the right modelling decisions but could reliably translate natural language instructions to API calls, it would find \plan an easier task. However, we find that a more explicit plan doesn't consistently boost performance. We hypothesize this could be due to  the LLM hallucinating API calls by following natural language instructions verbatim. For instance, for Heat Transfer problems, that accounts for a considerable fraction of problems, the natural language instructions in \plan instruct the LM to construct a `Heat Transfer in Solids' interface. However, the correct syntactical name of the interface is \texttt{HeatTransfer}. This is also observable in the slight drop on Interface Factuality between the two tasks in \tref{tab:compare_ongem2}. \textit{Grounding the LLM with information about or interaction with the API boosts performance.} PhyDoc In-Context reduces interface hallucinations for both tasks (factuality: 0.54$\rightarrow$1.0, 0.38$\rightarrow$0.85).

\begin{figure}[h]
\includegraphics[width=\textwidth]{figs/tool_demo_upd.pdf}
\caption{The Evaluator's feedback (\textit{left}) is passed to the ToolLookupAgent, that calls \textbf{\textit{tools}} and returns their concatenated output. {\color{lm} \textbf{Violet}}, on the \textit{left} indicates that the Verifier Feedback is returned by an LLM, and on the \textit{right}, denotes the arguments chosen by the ToolLookupAgent to call the tools with. The numerical annotations highlight the correspondence between the errors and arguments.}
\label{fig:tool_demo}
\end{figure}

\subsection{Agent Results}
 The interactive Multi-Turn Agent has the highest performance of all experiments on the \model task across several metrics including executability \change{(0.62 $\rightarrow$0.88)}. \fref{fig:blockwise} analyzes the executability across the initial `population' of LLM solutions generated for the problems by breaking down line-wise executability by the block of code the line belongs to. The physics block is the most challenging to generate executable code given a single query, motivating our focus on evaluation metrics that focus on
the physics block and tools that seek to help ground the LLM's code with physics-specific information. Over the course of its trajectory, the agent proposes 40 solutions: 20 from oversampling the initial prompt, and another 20 from correcting the best of the initial 20, and the best solution is selected from the tracked best solutions. This allows us to include gains obtained both from oversampling as well as from correction. For 5 problems, the best solution corresponded to one of the initial population of solutions.

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figs/blockwise15.png}
\caption{Block-wise executability across 300 samples of code with PhyDoc In-Context and Gemini-1.5-Pro. The physics block has the lowest executability. Error bars denote standard \mbox{deviations}.}
\label{fig:blockwise}
\end{figure} 

Although \textbf{Relative Error $|$ Strict} is the principal metric one would ideally want to optimize for, we do not report means over that metric here since the LLM was only able to compute a Valid Target that was also within 10\% of the correct answer for a single problem in the Multi-Turn Agent and ModelSpecs + PhyDoc experiments. For this problem, the correct target value is 18.3$^\circ$ Celsius, and the value exported by the LLM is 20$^\circ$ Celsius, which is a default temperature in \comsol: this is an indicator of the solution not being solved correctly. While a stricter relative error threshold would filter out such serendipitous matches, this risks filtering out problems in which a solution might be conceptually correct but differs from the target because of say, differences in solver and mesh sizes. \textit{The inability of the agent to correctly solve any of these problems attests to the challenge of the task and the need for additional research in this area to devise systems that are able to solve such problems.} 
}

==> workshop_contents/owa_results.tex <==
\input{workshop_contents/benchmain_only_res}
\input{workshop_contents/owa_longerres}

==> workshop_contents/results.tex <==
\input{workshop_contents/benchmain_only_res}

\paragraph{Comparison across Tasks and Agent Settings} We fix the LLM to Gemini-1.5-Pro, and compare performance with the list of physics interfaces and features (PhyDoc In-Context) added to the prompt and in an interactive multi-turn agent setting. The agent is equipped with an `evaluator' that both executes the code and records API replies and when executability crosses 90\%, examines the code and the output table, and returns feedback, in an `LLM-as-Judge' fashion. It thus computes a `fitness' for each solution \textit{without} having access to the GT target value. The fitness is used to track the best solutions. The \textsc{ControllerAgent} calls a \textsc{CorrectorSubAgent} that calls tools that aid it in correcting the code given the `current' code and feedback, execution history and the result of tool calls. An initial set of 20 samples are generated using PhyDoc In-Context and the best solutions are corrected for 20 steps (see \aref{app:agent} for details). The best of all solutions is then identified and evaluated. Both PhyDoc In-Context and the agentic setting \cready{significantly reduce} interface hallucinations, and the agent's mean executability is \cready{0.88 (vs 0.62). \textit{Thus, grounding the LLM with information about or interaction with the API boosts performance}. This indicates that at least some of the difficulty the LLMs encounter is due to their lack of knowledge of valid arguments to the API commands. We further examine whether the \plan task is easier. The comparison between task versions is of interest since both demand slightly different skills.}
\begin{wrapfigure}[20]{r}{0.4\textwidth}
    \centering
    \includegraphics[width=0.4\textwidth]{figs/blockwise15.png}
\caption{Block-wise executability on \cready{300} samples of code with PhyDoc In-Context and Gemini-1.5-Pro. The physics block has the lowest executability. Error bars are standard \mbox{deviations}.}
\label{fig:blockwise}
\end{wrapfigure} 
\cready{
For a person attempting to solve this task, \model requires the individual to both \textit{infer }implicit engineering and physical reasoning decisions to be made (e.g.: the LLM needs to infer that the correct representation of a cylinder's 2D cross-section is a rectangle) and further translate this to valid API calls. \plan explicitly describes all steps to be followed in natural language and requires the LLM to only \textit{translate} the steps describing interactions with the GUI to valid calls. The comparison between the two tasks offers one way to decouple the complexity of making correct modelling decisions from the difficulty of translating decisions into syntactically correct API calls. If an LLM fared poorly at making the right modelling decisions but could reliably translate natural language instructions to API calls, it would find \plan an easier task. However, we find that a more explicit plan doesn't consistently boost performance. Although \textbf{Relative Error $|$ Strict} is the principal metric one would ideally want to optimize for, we do not report means over that metric here since the LLM was only able to compute a Valid Target that was also within 10\% of the correct answer for a single problem in the Multi-Turn Agent and ModelSpecs + PhyDoc experiments. For this problem, the correct target value is 18.3$^\circ$ Celsius, and the value exported by the LLM is 20$^\circ$ Celsius, which is a default temperature in \comsol: this is an indicator of the solution not being solved correctly. While a stricter relative error threshold would filter out such serendipitous matches, this risks filtering out problems in which a solution might be conceptually correct but differs from the target because of say, differences in solver and mesh sizes. In \fref{fig:blockwise}, we used the initial population of samples generated by the LLMs to analyze executability within different blocks of code. The physics block has the lowest executability, thus motivating our focus on metrics that seek to measure performance on the physics decisions (API calls) made by the LLM. }

==> workshop_contents/shared_ack.tex <==
We are grateful to Eser Aygün for valuable suggestions on agent design. We thank Stephan Hoyer and Marc Coram for useful comments on the draft, and are grateful to Lizzie Dorfman and Rachel Stigler for their guidance. At Harvard, NM is partially supported by the National Science Foundation under Cooperative Agreement PHY2019786 (The NSF AI Institute for Artificial Intelligence and Fundamental Interactions).

==> workshop_contents/supp_math-ai.tex <==
\section{Dataset Curation}
\label{A: Dataset}
\input{supp/supp_bench_wksp}

% \todo{Add list of problems?}
\section{Evaluation Details}
\label{A: Eval}
\input{supp/eval}

\section{Querying the \comsol API from Python}
\subsection{The Python-\comsol Bridge}
\label{app:mph}
The raw output of the LLM is a string containing \comsol API commands in Java. An interface between Python and \comsol is needed to execute this code and interact in other ways with the API. We use the Python package MPh \citep{mph} and Rpyc for this. MPh is a scripting interface built on JPype \citep{jp} that enables a Python program to communicate with and build a model in \comsol. Each Java API command in the LM's output can be `pythonized' algorithmically. In most cases, the pythonized line is near identical to the Java line. However, due to differences in Java and Python syntax there exist some corner cases that need to be handled separately. Eg: `new String[]' is exclusively a Java construction, while the notation for booleans in Python is True / False as opposed to true / false in Java. Thus a `pythonizer' is constructed that parses and translates Java API calls to their Python counterparts.

The setup involves the following assumptions: an MPh client object is created. This behaves like a stateful `sandbox', where models can be built by LLMs, code can be evaluated, or information such as the current state of the model tree, properties under a node and the exported table can be queried and retrieved. Although multiple models can be created and set under the client, for simplicity we work with settings that involve a single model. Before running a new solution, the existing model is deleted and a new blank model is created. The LLM actions will modify this blank model. Thus, by design, all lines of code the LLM outputs, should start with `\texttt{model.}' and end with `;'.

\subsection{\comsol Code Structure}
\label{app: codeblocks}
\begin{enumerate}
    \item \textit{Geometry}, if any: This involves identifying the dimensionality of the problem, and constructing a representation of the object being modelled, say a cup, by creating and composing primitive shapes such as ellipses or rectangles to build the object. While already constructed geometries can also be imported from other software such as CAD, in our benchmark, we currently restrict ourselves to models for which we construct the geometry from scratch in COMSOL. This typically starts with a `model.component(``comp1").geom' pattern.
    \item \textit{Physics}: This will include specifying all the physical conditions for the problem, including initial or boundary conditions, forces, properties or in the case of mathematics problems, the differential equation. This typically starts with a `model.component(``comp1").physics' pattern. Some problems may additionally have lines that begin with `model.component(``comp`).multiphysics`, and set up the coupling between different kinds of physical phenomena. We categorize these lines, if any as `physics' in \fref{fig:blockwise}.
    
    \item \textit{Material}: Creating materials and assigning them to domains. One can either assign known materials such as `Copper' and the object will inherit the default properties of that material, or define a blank material and its properties such as conductivity from scratch. This typically starts with a `model.component(``comp1").material' pattern.
    \item \textit{Mesh}: Usually a shorter step that involves meshing the surfaces of the geometry to set up elements. This typically starts with a `model.component(``comp1").mesh' pattern.
    \item \textit{Study / Solver:} This involves specifying the conditions of the analysis and solver, such as the number of timesteps. While the solver code can be modified to override defaults, COMSOL also has the ability to automatically populate the model with the default solvers most apt for a given problem. This typically starts with a `model.study' or `model.sol' pattern respectively. In \fref{fig:blockwise}, we categorize both patterns as `solver'.
    \item \textit{Results:} Once the numerical solver has completed the analysis, one will likely postprocess the problem, in order to generate desired plots or tables. This typically starts with a `model.result' pattern.
\end{enumerate}


\label{app:agent}
\ifthenelse{\boolean{owa}}{% Do nothing if false
}{%math-ai
\section{Agent Design}
\input{iclr_contents/agent_methods}
\begin{figure}[h]
\includegraphics[width=\textwidth]{figs/tool_demo_upd.pdf}
\caption{The Evaluator's feedback (\textit{left}) is passed to the ToolLookupAgent, that calls \textbf{\textit{tools}} and returns their concatenated output. {\color{lm} \textbf{Violet}}, on the \textit{left} indicates that the Verifier Feedback is returned by an LLM, and on the \textit{right}, denotes the arguments chosen by the ToolLookupAgent to call the tools with. The numerical annotations highlight the correspondence between the errors and arguments.}
\label{fig:tool_demo}
\end{figure}
}

\section{Agent Details}
\input{supp/shared_agent_details}


\section{Qualitative Analysis}
\label{app:qual}
\input{workshop_contents/analysis}
\newpage


\section{Prompts}
\label{app: prompts}
\input{iclr_contents/app_prompts}
% \subsection{Dataset Generation Prompts}
